Design under Throughput Scale-Up: Equations that Transfer the Pressure-Conversion Front to Untested Flow Rates in a Reactive Tesla-Valve Micromixer

Raising the flow rate through a reactive micromixer shortens residence time and raises pressure drop, so a geometry chosen at one flow rate may not suit another, and repeating a CFD optimisation at every flow rate is costly. We test whether short equations fitted across optimisation campaigns recover the pressure-conversion front at a flow rate that was not optimised. A Tesla-valve micromixer running the Bourne neutralisation-hydrolysis reactions was optimised by multi-fidelity Bayesian optimisation at seven velocities over an eightfold range. Symbolic regression of the seven surrogates, with no functional form imposed, returned the same equations in three independent searches: pressure drop is a hydraulic resistance proportional to flow rate, and the effective Damk\"ohler number is set by a channel length divided by flow rate, a contact time. A diffusion-only estimate reproduces the fine-mesh conversion, so in this two-dimensional laminar model the stages act through contact time rather than added mixing, and the efficient geometries change little with flow rate. Equations of 12 nodes found without one flow rate placed the front there within 0.5 percentage points of conversion and kept 95% of its hypervolume; longer equations fitted better without predicting better fronts. Twenty new fine-mesh designs taken from predicted fronts confirmed the accuracy of the equations and the size of that shortfall. Inside the range already sampled, a fine-mesh check of a few designs read from the equations, about two hours of CFD, replaces a new optimisation of about 40 hours. For the Tesla valve, the highest conversion fell by half across the flow range, and keeping conversion while doubling the flow rate per channel requires twice the device length and about four times the pressure drop.

==> figures/figure01_icons_lib.tex <==
\providecommand{\icc}{black}\providecommand{\ica}{black}\providecommand{\icb}{white}
\providecommand{\icf}{black!15}\providecommand{\icp}{orange!85!black}
\providecommand{\chf}{black!12}\providecommand{\che}{black}
\providecommand{\lamA}{\icc}\providecommand{\lamB}{\icc}\providecommand{\lamC}{\icc}
\newcommand{\icondesign}{%
  \begin{scope}[scale=0.82]
  \def\tpath{(-0.70,0.22) -- (-0.54,0.0) (-0.70,-0.22) -- (-0.54,0.0) (-0.54,0.0) -- (0.70,0.0)
             (-0.46,0.0) .. controls (-0.36,0.40) and (-0.06,0.44) .. (0.04,0.20) .. controls (0.08,0.10) and (0.06,0.04) .. (0.0,0.0)
             (0.10,0.0) .. controls (0.20,-0.40) and (0.50,-0.44) .. (0.60,-0.20) .. controls (0.64,-0.10) and (0.62,-0.04) .. (0.56,0.0)}
  \draw[line width=3.2pt, \che, line cap=butt, line join=round] \tpath;
  \draw[line width=2.0pt, \chf, line cap=butt, line join=round] \tpath;
  \draw[-{Latex[length=1.2mm]}, line width=0.6pt, \ica] (-0.62,0.52) -- (-0.50,0.30);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=east] at (-0.62,0.52) {$\lambda$};
  \end{scope}}
\newcommand{\icondesignB}{%
  \begin{scope}[scale=0.80]
  \def\tpath{(-0.72,0.20) -- (-0.58,0.0) (-0.72,-0.20) -- (-0.58,0.0) (-0.58,0.0) -- (0.72,0.0)
             (-0.52,0.0) .. controls (-0.46,0.36) and (-0.20,0.38) .. (-0.14,0.18) .. controls (-0.12,0.08) and (-0.14,0.03) .. (-0.18,0.0)
             (-0.12,0.0) .. controls (-0.06,-0.36) and (0.20,-0.38) .. (0.26,-0.18) .. controls (0.28,-0.08) and (0.26,-0.03) .. (0.22,0.0)
             (0.28,0.0) .. controls (0.34,0.36) and (0.60,0.38) .. (0.66,0.18) .. controls (0.68,0.08) and (0.66,0.03) .. (0.62,0.0)}
  \draw[line width=3.0pt, \che, line cap=butt, line join=round] \tpath;
  \draw[line width=1.8pt, \chf, line cap=butt, line join=round] \tpath;
  \draw[-{Latex[length=1.2mm]}, line width=0.6pt, \ica] (-0.62,0.52) -- (-0.52,0.28);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=east] at (-0.62,0.52) {$\lambda$};
  \end{scope}}
\newcommand{\icondesignE}[1]{%
  \node[inner sep=0pt] at (0.04,0.02) {\includegraphics[width=1.24cm]{#1}};
  \draw[-{Latex[length=1.2mm]}, line width=0.6pt, \ica] (-0.36,0.40) -- (-0.44,0.18);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=south west, inner sep=1pt] at (-0.38,0.36) {$\lambda$};
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=north, inner sep=1pt] at (0.40,-0.24) {$\times N$};}
\newcommand{\icondesignF}[1]{%
  \node[inner sep=0pt] at (0,0.09) {\includegraphics[width=1.18cm]{#1}};
  \draw[-{Latex[length=1.1mm]}, line width=0.6pt, \ica] (-0.48,-0.30) -- (-0.22,-0.30);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=east, inner sep=1pt] at (-0.48,-0.30) {$\lambda$};
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, inner sep=1pt] at (0.32,-0.30) {$\times N$};}
\newcommand{\icondesignG}[1]{%
  \begin{scope}[yshift=-0.04cm]
  \node[inner sep=0pt] at (0.04,0.02) {\includegraphics[width=1.24cm]{#1}};
  \draw[-{Latex[length=1.1mm]}, line width=0.6pt, \ica] (-0.40,0.44) -- (-0.29,0.10);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=south, inner sep=1pt] at (-0.42,0.42) {$\lambda$};
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=north east, inner sep=1pt] at (0.64,-0.07) {$\times N$};
  \end{scope}}
\newcommand{\icondesignH}[1]{%
  \begin{scope}[yshift=-0.03cm]
  \node[inner sep=0pt] at (0.10,0.02) {\includegraphics[width=1.12cm]{#1}};
  \draw[-{Latex[length=1.1mm]}, line width=0.6pt, \ica] (-0.66,0.02) -- (-0.47,0.02);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=south, inner sep=1pt] at (-0.60,0.05) {$\lambda$};
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=north east, inner sep=0.5pt] at (0.64,-0.06) {$\times N$};
  \end{scope}}
\newcommand{\icondesignI}[1]{%
  \begin{scope}[yshift=-0.03cm]
  \node[inner sep=0pt] at (0.08,0.02) {\includegraphics[width=1.20cm]{#1}};
  \draw[-{Latex[length=1.1mm]}, line width=0.6pt, \ica] (-0.68,0.13) -- (-0.50,-0.01);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=south east, inner sep=0.5pt] at (-0.66,0.13) {$\lambda$};
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=north east, inner sep=0.5pt] at (0.66,-0.06) {$\times N$};
  \end{scope}}
\newcommand{\icondesignJ}[1]{%
  \begin{scope}[yshift=-0.04cm]
  \node[inner sep=0pt] at (0.04,0.02) {\includegraphics[width=1.30cm]{#1}};
  \draw[-{Latex[length=1.1mm]}, line width=0.6pt, \ica] (-0.42,0.46) -- (-0.33,0.18);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=south, inner sep=1pt] at (-0.44,0.44) {$\lambda$};
  \node[font=\fontsize{7}{8}\selectfont, text=\icc, anchor=north east, inner sep=0.5pt] at (0.66,-0.08) {$\times N$};
  \end{scope}}
\newcommand{\iconmesh}{%
  \begin{scope}[scale=0.80]
  \foreach \xo/\n in {-0.64/1, -0.20/2, 0.24/4}{
    \draw[line width=0.6pt, \icc] (\xo,-0.24) rectangle ++(0.40,0.40);
    \pgfmathsetmacro{\stp}{0.40/\n}
    \foreach \k in {1,...,\n}{
      \draw[line width=0.28pt, \icc] (\xo+\k*\stp,-0.24) -- ++(0,0.40);
      \draw[line width=0.28pt, \icc] (\xo,-0.24+\k*\stp) -- ++(0.40,0);}}
  \fill[\icc] (-0.56,0.25) circle (0.04) (-0.44,0.25) circle (0.04) (-0.32,0.25) circle (0.04)
              (-0.06,0.25) circle (0.04) (0.06,0.25) circle (0.04) (0.44,0.25) circle (0.04);
  \draw[-{Latex[length=1.2mm]}, line width=0.6pt, \ica] (-0.58,-0.42) -- (0.58,-0.42);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc] at (0.0,-0.56) {$z$};
  \end{scope}}
\newcommand{\iconmeshcont}{%
  \begin{scope}[scale=0.85]
  \draw[line width=0.6pt, \icc] (-0.62,-0.30) rectangle (0.62,0.22);
  \foreach \x in {-0.40,-0.22,-0.07,0.05,0.15,0.235,0.305,0.365,0.415,0.46,0.50,0.535,0.565,0.59}{
    \draw[line width=0.28pt, \icc] (\x,-0.30) -- (\x,0.22);}
  \foreach \y in {-0.17,-0.04,0.09}{\draw[line width=0.28pt, \icc] (-0.62,\y) -- (0.62,\y);}
  \draw[-{Latex[length=1.2mm]}, line width=0.6pt, \ica] (-0.58,-0.46) -- (0.58,-0.46);
  \node[font=\fontsize{7}{8}\selectfont, text=\icc] at (0.0,-0.60) {$z$};
  \end{scope}}

\newcommand{\icondesignK}[1]{%
  \node[inner sep=0pt] at (0,0) {\includegraphics[width=1.36cm]{#1}};}
\newcommand{\iconaxes}{%
  \draw[-{Latex[length=1.1mm]}, line width=0.6pt, \icc] (-0.58,-0.52) -- (0.64,-0.52);
  \draw[-{Latex[length=1.1mm]}, line width=0.6pt, \icc] (-0.58,-0.52) -- (-0.58,0.58);}
\newcommand{\iconfront}{%
  \begin{scope}[scale=0.88]\iconaxes
  \draw[line width=0.9pt, \lamA] (-0.48,-0.10) .. controls (-0.38,0.30) and (-0.10,0.42) .. (0.10,0.46);
  \draw[line width=0.9pt, \lamB] (-0.40,-0.30) .. controls (-0.22,0.10) and (0.05,0.20) .. (0.32,0.24);
  \draw[line width=0.9pt, \lamC] (-0.30,-0.44) .. controls (-0.08,-0.10) and (0.20,0.00) .. (0.54,0.02);
  \fill[\lamA] (-0.48,-0.10) circle (0.05) (-0.24,0.33) circle (0.05) (0.10,0.46) circle (0.05);
  \fill[\lamB] (-0.40,-0.30) circle (0.05) (-0.08,0.13) circle (0.05) (0.32,0.24) circle (0.05);
  \fill[\lamC] (-0.30,-0.44) circle (0.05) (0.08,-0.06) circle (0.05) (0.54,0.02) circle (0.05);\end{scope}}
\newcommand{\icongp}{%
  \begin{scope}[scale=0.88]
  \fill[\icf] (-0.56,-0.22) .. controls (-0.22,0.48) and (0.05,-0.32) .. (0.56,0.38)
              -- (0.56,0.02) .. controls (0.05,-0.62) and (-0.22,0.12) .. (-0.56,-0.52) -- cycle;
  \draw[line width=0.9pt, \icc] (-0.56,-0.37) .. controls (-0.22,0.30) and (0.05,-0.47) .. (0.56,0.20);
  \fill[\icc] (-0.36,-0.10) circle (0.055) (-0.02,-0.13) circle (0.055) (0.36,0.03) circle (0.055);
  \end{scope}}
\newcommand{\icontree}{%
  \begin{scope}[scale=0.72, yshift=0.06cm]
  \draw[line width=0.7pt, \icc] (0,0.46) -- (-0.36,0.0) (0,0.46) -- (0.36,0.0) (-0.36,0.0) -- (-0.62,-0.46) (-0.36,0.0) -- (-0.10,-0.46);
  \tikzset{tn/.style={draw=\icc, fill=\icb, circle, inner sep=0pt, minimum size=0.25cm, font=\fontsize{7}{8}\selectfont, line width=0.6pt, text=\icc}}
  \node[tn] at (0,0.46) {$\div$};
  \node[tn] at (-0.36,0.0) {$+$};
  \node[tn] at (0.36,0.0) {$\lambda$};
  \node[tn] at (-0.62,-0.46) {$N$};
  \node[tn] at (-0.10,-0.46) {$p$};
  \end{scope}}
\newcommand{\iconwithheld}{%
  \begin{scope}[scale=0.85]\iconaxes
  \draw[line width=0.7pt, \lamA] (-0.48,-0.10) .. controls (-0.38,0.30) and (-0.10,0.42) .. (0.10,0.46);
  \draw[line width=0.7pt, \lamC] (-0.30,-0.44) .. controls (-0.08,-0.10) and (0.20,0.00) .. (0.54,0.02);
  \draw[line width=0.7pt, \icp, dash pattern=on 1.0pt off 0.55pt]
    (-0.42,-0.32) -- (-0.30,-0.32) -- (-0.30,-0.06) -- (-0.12,-0.06) -- (-0.12,0.10) -- (0.08,0.10) -- (0.08,0.18) -- (0.16,0.18);
  \node[font=\fontsize{7}{8}\selectfont, text=\icp, anchor=west, inner sep=1pt] at (0.16,0.19) {$\lambda^\star$};
  \end{scope}}
\newcommand{\iconnewcfd}{%
  \begin{scope}[scale=0.88]\iconaxes
  \draw[line width=1.1pt, \icp, dash pattern=on 1.0pt off 0.55pt] (-0.44,-0.36) .. controls (-0.28,0.14) and (0.06,0.30) .. (0.42,0.355);
  \node[star, star points=5, star point ratio=2.4, fill=\icc, inner sep=0pt, minimum size=0.26cm] at (-0.30,-0.06) {};
  \node[star, star points=5, star point ratio=2.4, fill=\icc, inner sep=0pt, minimum size=0.26cm] at (0.02,0.20) {};
  \node[star, star points=5, star point ratio=2.4, fill=\icc, inner sep=0pt, minimum size=0.26cm] at (0.38,0.33) {};\end{scope}}
\newcommand{\iconclock}{%
  \begin{scope}[scale=0.85]
  \draw[line width=0.65pt, \icc] (0,-0.08) circle (0.44);
  \draw[line width=0.8pt, \icc] (0,0.36) -- (0,0.46);
  \draw[line width=1.0pt, \icc, line cap=round] (-0.12,0.50) -- (0.12,0.50);
  \fill[\icf] (0,-0.08) -- (0,0.30) arc (90:-30:0.38) -- cycle;
  \draw[line width=1.0pt, \icc, line cap=round] (0,-0.08) -- (0,0.24);
  \draw[line width=1.0pt, \icc, line cap=round] (0,-0.08) -- (0.22,-0.20);
  \fill[\icc] (0,-0.08) circle (0.04);\end{scope}}

